Conformal Mixed-Integer Constraint Learning with Feasibility Guarantees

We propose Conformal Mixed-Integer Constraint Learning (C-MICL), a novel framework that provides probabilistic feasibility guarantees for data-driven constraints in optimization problems. While standard Mixed-Integer Constraint Learning methods often violate the true constraints due to model error or data limitations, our C-MICL approach leverages conformal prediction to ensure feasible solutions are ground-truth feasible. This guarantee holds with probability at least $1{-}\alpha$, under a conditional independence assumption. The proposed framework supports both regression and classification tasks without requiring access to the true constraint function, while avoiding the scalability issues associated with ensemble-based heuristics. Experiments on real-world applications demonstrate that C-MICL consistently achieves target feasibility rates, maintains competitive objective performance, and significantly reduces computational cost compared to existing methods. Our work bridges mathematical optimization and machine learning, offering a principled approach to incorporate uncertainty-aware constraints into decision-making with rigorous statistical guarantees.

==> proofs.tex <==
\newpage

%\begin{theorem} [PAC ground-truth feasibility guarantee for C-MICL Optimal Solutions] Let $x^*(D_{\text{cal}})$ denote the optimal solution to the C-MICL problem for a given iid calibration dataset $D_{\text{cal}}$ of size $N$. For any $\delta \in (0,1)$, with probability at least $1-\delta$ over random draws of $D_{\text{cal}}$, the optimal solution satisfies:
%$$\mathbb{P}(h(x^*(D_{\text{cal}})) \in \mathcal{Y} \mid D_{\text{cal}}) \geq 1 - \alpha - \sqrt{\frac{\log(1/\delta)}{2N}}$$
    
%\end{theorem}

%\begin{proof}
%By Vovk [2012, Proposition 2a], for any independent test point $x$, the conformal prediction set $\mathcal{C}(x)$ satisfies the \textit{training-conditional} coverage:
% $$\mathbb{P}_{D_{\text{cal}}}\left(\mathbb{P}(h(x) \in \mathcal{C}(x) \mid D_{\text{cal}}) \geq 1-\alpha-\epsilon\right) \geq 1-\delta$$
%where $\epsilon = \sqrt{\frac{\log(1/\delta)}{2N}}$ is derived from Hoeffding's inequality.


%The key challenge in applying this result to the optimal solution $x^*(D_{\text{cal}})$ is that it is not independent of $D_{\text{cal}}$. Nevertheless, while $x^*(D_{\text{cal}})$ depends on $D_{\text{cal}}$, this dependency is through the optimization  objective and the constraint $\mathcal{C}(x) \subseteq \mathcal{Y}$, which doesn't directly exploit the relationship between $h(x)$ and $\mathcal{C}(x)$. That is, the optimization procedure is ``blind'' to whether $h(x) \in \mathcal{C}(x,D_{\text{cal}})$ for any particular $x$: the optimization criterion is independent of the event $\{h(x) \in \mathcal{C}(x,D_{\text{cal}})\}$. This property ensures that the probability guarantee from conformal prediction remains valid despite the dependency.

%In particular, for the optimal solution $x^*(D_{\text{cal}})$, the conformal set provides conditional coverage $\PP(h(x^*(D_{\text{cal}})) \in \mathcal{C}(x^*(D_{\text{cal}})) \mid \mathcal{D}_{\text{cal}})$ of at least $1-\alpha-\epsilon$ with probability at least $1-\delta$ over draws of $D_{\text{cal}}$,

%By construction of the C-MICL problem, for any realization of $D_{\text{cal}}$, the optimal solution $x^*(D_{\text{cal}})$ satisfies $\mathcal{C}(x^*(D_{\text{cal}})) \subseteq \mathcal{Y}$. This implies that whenever $h(x^*(D_{\text{cal}})) \in \mathcal{C}(x^*(D_{\text{cal}}))$, we must also have $h(x^*(D_{\text{cal}})) \in \mathcal{Y}$. 

%Combining these results, with probability at least $1-\delta$ over draws of $D_{\text{cal}}$:
%$$\begin{aligned}
%\mathbb{P}(h(x^*(D_{\text{cal}})) \in \mathcal{Y} \mid D_{\text{cal}}) &\geq \mathbb{P}(h(x^*(D_{\text{cal}})) \in \mathcal{C}(x^*(D_{\text{cal}})) \mid D_{\text{cal}}) \\
%&\geq 1-\alpha-\sqrt{\frac{\log(1/\delta)}{2N}}
%\end{aligned}$$
%which establishes the desired PAC guarantee for ground-truth feasibility of the optimal solution.
%\end{proof}


\begin{assumption}
    \textbf{(Conformal Coverage Invariance)}: Let $\mathcal{F}_N = \{(x,z) \in \mathcal{X}: g(x,z)\leq 0, \mathcal{C}(x) \subseteq \mathcal{Y}\}$ be the feasible region of the C-MICL problem. The coverage property of conformal prediction sets is preserved when considering only points that satisfy the C-MICL constraint. Formally:
$$\mathbb{P}(h(x) \in \mathcal{C}(x) \mid (x,z) \in \mathcal{F}_N) \geq 1-\alpha$$
\end{assumption}

\begin{theorem}
    Under Assumption 1, any feasible solution $(x', z')$ of the C-MICL problem is ground-truth feasible with probability:
\begin{equation}
\mathbb{P}\left( h(x') \in \mathcal{Y} \mid (x', z') \in \mathcal{F}_N \right) \geq 1-\alpha,
\end{equation}
for a pre-specified target coverage level $1{-}\alpha$.
\end{theorem}


\begin{proof}
     From the \ref{eq:c-micl} formulation, when a solution $(x', z')$ is feasible we know that $\mathcal{C}(x') \subseteq \mathcal{Y}$. Moreover, by Assumption 1, for feasible points we have that the true function value $h(x')$ falls within $\mathcal{C}(x')$ with probability at least $1{-}\alpha$. Since $\mathcal{C}(x')$ is a subset of $\mathcal{Y}$, whenever $h(x')$ is in $\mathcal{C}(x')$, it must also be in $\mathcal{Y}$. Therefore, $\mathbb{P}(h(x') \in \mathcal{Y}) \geq \mathbb{P}(h(x') \in \mathcal{C}(x')) \geq 1{-}\alpha$, which proves the ground-truth feasibility guarantee for any feasible solution to the  \ref{eq:c-micl} problem.
\end{proof}



\textbf{Assumption 2 (Label-Conditional Conformal Coverage Guarantee)}: The coverage property of conformal prediction sets is preserved for ground truth feasible and not feasible points:
$$P(h(x) \in C(x) \mid h(x) \in \mathcal{Y}) \geq 1-\alpha$$
$$P(h(x) \in C(x) \mid h(x) \notin \mathcal{Y}) \geq 1-\alpha$$

\textbf{Assumption 3 (Conditional Independence of Feasibility and Coverage)}: The events of feasibility and conformal coverage are conditionally independent given $h(x)$.


Proof de lo que queremos:

By law of total probability:

\begin{align*}
    P(h(x) \in C(x) \mid x \in F)  = & P(h(x) \in C(x) \mid x \in F, h(x) \in \mathcal{Y})*P(h(x) \in \mathcal{Y} \mid x \in F) \\
    & + P(h(x) \in C(x) \mid x \in F, h(x) \notin \mathcal{Y})*P(h(x) \notin \mathcal{Y} \mid x \in F) \\
    = &  P(h(x) \in C(x) \mid h(x) \in \mathcal{Y})*P(h(x) \in \mathcal{Y} \mid x \in F) \\
    & + P(h(x) \in C(x) \mid h(x) \notin \mathcal{Y})*P(h(x) \notin \mathcal{Y} \mid x \in F) \\
    \geq & (1-\alpha)*P(h(x) \in \mathcal{Y} \mid x \in F) + (1-\alpha)*P(h(x) \notin \mathcal{Y} \mid x \in F) \\
    = &  (1-\alpha)*[P(h(x) \in \mathcal{Y} \mid x \in F) + P(h(x) \notin \mathcal{Y} \mid x \in F) ] \\
    = &  (1-\alpha)
\end{align*}


$P(h(x) \in C(x) \mid x \in F, h(x) \in \mathcal{Y}) = P(h(x) \in C(x) \mid h(x) \in \mathcal{Y})$

\newpage

\begin{proof}

\begin{align*}
    P(h(x) \in C(x) \mid x \in F)  = & P(h(x) \in C(x) \mid x \in F, h(x) \in \mathcal{Y})*P(h(x) \in \mathcal{Y} \mid x \in F) \\
    & + P(h(x) \in C(x) \mid x \in F, h(x) \notin \mathcal{Y})*P(h(x) \notin \mathcal{Y} \mid x \in F) \\
    = &  P(h(x) \in C(x) \mid h(x) \in \mathcal{Y})*P(h(x) \in \mathcal{Y} \mid x \in F) \\
    & + P(h(x) \in C(x) \mid h(x) \notin \mathcal{Y})*P(h(x) \notin \mathcal{Y} \mid x \in F) \\
    \geq & (1-\alpha)*P(h(x) \in \mathcal{Y} \mid x \in F) + (1-\alpha)*P(h(x) \notin \mathcal{Y} \mid x \in F) \\
    = &  (1-\alpha)*[P(h(x) \in \mathcal{Y} \mid x \in F) + P(h(x) \notin \mathcal{Y} \mid x \in F) ] \\
    = &  (1-\alpha)
\end{align*}

where the probability is taken with respect to both the calibration data $\mathcal{D}_\text{cal}$ and the test point $(x', z')$.

     From the \ref{eq:c-micl} formulation, when a solution $(x', z')$ is feasible we know that $\mathcal{C}(x') \subseteq \mathcal{Y}$. Moreover, by \Cref{thm:cp_quantile}, the true function value $h(x')$ falls within $\mathcal{C}(x')$ with probability at least $1{-}\alpha$. Since $\mathcal{C}(x')$ is a subset of $\mathcal{Y}$, whenever $h(x')$ is in $\mathcal{C}(x')$, it must also be in $\mathcal{Y}$. Therefore, $\mathbb{P}(h(x') \in \mathcal{Y}) \geq \mathbb{P}(h(x') \in \mathcal{C}(x')) \geq 1{-}\alpha$, which proves the ground-truth feasibility guarantee.
\end{proof}

